Linguini: A benchmark for language-agnostic linguistic reasoning

We propose a new benchmark to measure a language model's linguistic reasoning skills without relying on pre-existing language-specific knowledge. The test covers 894 questions grouped in 160 problems across 75 (mostly) extremely low-resource languages, extracted from the International Linguistic Olympiad corpus. To attain high accuracy on this benchmark, models don't need previous knowledge of the tested language, as all the information needed to solve the linguistic puzzle is presented in the context. We find that, while all analyzed models rank below 25% accuracy, there is a significant gap between open and closed models, with the best-performing proprietary model at 24.05% and the best-performing open model at 8.84%.

==> datacard.tex <==

% Optional: reduce margins single line to fit in "one to two pages", as recommended
%\begin{adjustwidth}{-5pt}{-2pt}
\begin{singlespace}
\newenvironment{mcsection}[1]
    {%
        \textbf{#1}

        % Reduce margins to use the space more effectively and help fit in the recommended "one to two pages"
        % Use the bullet list format as shown in the model card paper to increase readability
        \begin{itemize}%[leftmargin=*,topsep=0pt,itemsep=-1ex,partopsep=1ex,parsep=1ex,after=\vspace{\medskipamount}]
    }
    {%
        \end{itemize}
    }
\tcbset{colback=white!10!white}
\begin{tcolorbox}[title=\textbf{\section{Data Card for Linguini}},
    breakable, sharp corners, boxrule=0.5pt] 

% Change to a smaller, but still legible font size to help fit in the recommended "one to two pages"
\small{


\begin{mcsection}{Dataset Description\footnote{We use a template for this data card \url{https://huggingface.co/docs/datasets/v1.12.0/dataset_card.html} }} 
%\item Basic information about the model.
%\begin{itemize}

        \item Dataset Summary\\
\textit{Linguini dataset and benchmark measures a language model’s linguistic reasoning skills without relying on pre-existing language-specific knowledge. The test covers 894 questions grouped in 160 problems across 75 (mostly) extremely low-resource languages, extracted from the International Linguistic Olympiad corpus}
%\todo{Next table 1 summarizes the languages, source, total number of sentences and domains translated.}
\item How to use the data\\
You can access links to the data in the README {\color{red} at \url{add link}}
\item Supported Tasks and Leaderboards \\
\textit{Linguistic reasoning evaluation for language generation}
\item Languages\\
\textit{Linguini is currently available in English, but questions cover 75 low-resource languages.}
%\end{itemize}
\end{mcsection}


% \begin{mcsection}{Data Structure}
% %    \item Use cases that were envisioned during development.
% %\begin{itemize}
%     \item \textit{The dataset contains tab delimited text files for each direction. Each text file contains lines with parallel sentences.}

% \end{mcsection}




\begin{mcsection}{Dataset Creation}
 \item Curation Rationale\\
To select the types of questions for the dataset, we built a taxonomy exploring the IOL from 2003 to 2023. We excluded all instances for which their category only appears once; those where the question includes an image or those where the response is only an explanation. The remaining problems require solving different linguistic reasoning tasks, such as morphosyntactic segmentation (eg., verb conjugation), morphosemantic alignment (e.g., noun negation), derivation (e.g., finding cognates in related languages), morphophonological segmentation (e.g., pluralization) or graphophonemic transcription (e.g., transcription from one script to another). In total, Linguini is composed by questions grouped in 160 problems across 75 (mostly) extremely low-resource language. A list of languages can be found in Appendix \ref{tab:languages} in the paper.
\item Source Data\\
\textit{S
}

\item Annotations\\
\textit{Not applicable} 
\item Personal and Sensitive Information \\
 \textit{Not applicable}

\end{mcsection}


\begin{mcsection}{Considerations for Using the Data}
 %  \item Details on the dataset(s) used for the quantitative analyses in the card. \\
%\begin{itemize}
   \item Social Impact of Dataset\\
 \textit{This benchmark intends to address and quantify the root of multilingualism, which in turn can impact
the support of language models for the majority of world languages
} 
  \item Discussion of Biases\\
\textit{We have not studies any kind of biases in the dataset.}
 
 
\end{mcsection}

\begin{mcsection}{Additional Information}
 %  \item Details on the dataset(s) used for the quantitative analyses in the card. \\
\item Dataset Curators \\
\textit{Not applicable } 
 \item Licensing Information \\
 \textit{We are releasing under the terms of {\color{red} add dataset info}}%CC-BY-SA\footnote{\url{https://creativecommons.org/licenses/by-sa/4.0/}}}
 \item Citation Information\\
Sánchez et al, \textit{Linguini: A benchmark for language-agnostic
linguistic reasoning}, Submission to Neurips 2024
 %\todo{NLLB Team et al, \textit{No Language Left Behind:
%Scaling Human-Centered Machine Translation}, Arxiv, 2022}
 %\item Contributions(\#contributions)\\
%\todo{Cynthia Gao Elahe Kalbassi Janice Lam Christophe Ropers (?) }
 

\end{mcsection}





} % end font size change
\end{tcolorbox}
\end{singlespace}
\end{adjustwidth}
%\end{comment}



